Visual Servoing for Pose Control of Soft Continuum Arm in a Structured Environment

For soft continuum arms, visual servoing is a popular control strategy that relies on visual feedback to close the control loop. However, robust visual servoing is challenging as it requires reliable feature extraction from the image, accurate control models and sensors to perceive the shape of the arm, both of which can be hard to implement in a soft robot. This letter circumvents these challenges by presenting a deep neural network-based method to perform smooth and robust 3D positioning tasks on a soft arm by visual servoing using a camera mounted at the distal end of the arm. A convolutional neural network is trained to predict the actuations required to achieve the desired pose in a structured environment. Integrated and modular approaches for estimating the actuations from the image are proposed and are experimentally compared. A proportional control law is implemented to reduce the error between the desired and current image as seen by the camera. The model together with the proportional feedback control makes the described approach robust to several variations such as new targets, lighting, loads, and diminution of the soft arm. Furthermore, the model lends itself to be transferred to a new environment with minimal effort.

==> archive/Methods_old.tex <==
\subsection{Experimental setup}


\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{Figures/VS_SCA_exp_setup_v4.png}
    \caption{}
    \label{fig:exp_setup}
\end{figure*}
    \todo[inline]{I am sure this is too long, but I wrote it in detail and we can trim out as needed.}
       \todo[inline]{Should the Polhemus go here or is it fine where Naveen put it?}
    The experimental setup consists of four systems: SCA, gantry, electrical control board and computers.  The SCA is made of three Fiber Re-enforced Elastomeric Enclosures (FREE) - one bending, two rotational (CW and CCW) and is referred to as a BR2 actuator \cite{uppalapati2018}.  It has an individually controllable pneumatic actuator for each FREE.  The gantry (Figure \ref{fig:exp_setup}) adds three degrees of freedom to the SCA via an $X$ and $Y$ rail and a rotational mount ($\theta$) for the SCA.  This system is built from modular extruded aluminum (Actobotics U-Channel and X-Rail products, ServoCity).  The $X$ and $Y$ rails are belt driven by stepper motors (NEMA 17, Pololu) with limit switches setting the origin and end positions of each rail.   It has an $X$ travel of 45cm and a $Y$ travel of 42cm. Positioning on the gantry is open loop and must be periodically reset to reduce error accumulation.  $\theta$ is controlled by a servo motor (DS3218MG, DSSERVO) to which is fixed the SCA. This can rotate the SCA 90\degree{} in either direction and further expands the SCA's workspace \cite{uppalapati_valens}. Together the SCA and gantry provide five degrees of freedom: bending, rotation, theta, $X$ and $Y$ translation.  Note that rotation is treated as one DOF as the two rotating FREEs are never actuated simultaneously.  The CW and CCW rotations are distinguished by positive or negative value.
    
    The electrical control board contains:
    \begin{itemize}
        \item Pressure Regulators (ITV0031-2UBL, SMC) - Regulate the pressure to the SCA's FREEs
        \item Digital to Analog Converter (DAC)(MCP4728, Adafruit) - Provides the analog signal to the pressure regulators
        \item PWM Generator (PCA9685, Adafruit) - Controls the servo orientation
        \item Stepper Drivers (Big Easy Driver, SparkFun) - Controls the stepper motors
        \item Voltage Regulators - Provide the various required voltages
    \end{itemize}
    
    Two computers are used: A Raspberry Pi 4 (8Gb) and an Intel NUC (NUC7i7), both running Ubuntu 18.04 with ROS Melodic.  The Raspberry Pi is used to interface with the electrical control board and run all the associated hardware via ROS.  The NUC is used for the computationally intense visual servoing work.  The two systems are tied together via ROS multimaster.
    
   \subsection{Data collection}
    We  mounted  a  600  TVL  camera  which  is  a  low  cost camera with small form factor on the soft robotic arm mentioned earlier and collected images from the camera at various views by moving the soft arm.  The setup of the soft arm is given in Fig. The process is self-supervised and the inputs are given in the form of actuations, such as angle, base pressure. Images of  the  scenes  are  clicked  at  every  orientation. Few examples of images clicked by the camera mounted on the soft arm of the soft robot are shown in Fig \ref{fig:exp_setup} (f) and (g). The images are of resolution 640x480 pixels.

% \begin{figure}[htbp]
%   \centering
%   \begin{subfigure}[b]{0.42\textwidth}
%   \centering
%     \includegraphics[width=0.8\textwidth]{Figures/img2084.jpg}
%   \end{subfigure}
  
%   \begin{subfigure}[b]{0.42\textwidth}
%   \centering
%     \includegraphics[width=0.8\textwidth]{Figures/img2006.jpg}
%   \end{subfigure}
%   \caption{Images clicked by camera on soft arm}
%   \label{fig:data}
% \end{figure}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{Figures/Full_system_final.png}
    \caption{}
    \label{fig:Full system}
\end{figure*}
\subsection{Network Architecture}
Deep Convolutional Neural Networks have recently shown to be effective in various computer vision applications. Their ability to effortlessly extract features makes them a powerful tool in various image recognition tasks. CNNs have recently been studied to estimate the pose of a robot manipulator given image inputs \cite{8461068}. The motivation behind our approach is to use CNNs to estimate the input actuation values required to reach a specific pose of the soft manipulator arm using image inputs. \\
Transfer learning is a popular method of using pre-trained networks for tasks similar to the original task that the network was trained on. Fine-tuning can be applied to change certain aspects of the network to make it suitable for the new task at hand. Fine tuning also helps in case of smaller datasets such as ours where training from scratch may not guarantee good results. Since, in our approach, we use real-world images of scenes captured by the tip camera, a partially trained VGG16 network was used. The VGG16 network was trained on 1.2 million ImageNet images and has around 138 million parameters \cite{simonyan2014very}.\\
Since our task was not exactly similar to the original image classification task that VGG16 was trained on, we retrained some layers. This effectively helped the network to learn new features pertaining to our task, and update weights accordingly. We found that freezing the first 12 layers of the network and retraining the remaining layers gave optimal results in terms of loss and error. In addition to this, we added 3 fully connected layers (with 64, 32, 5 units respectively) with ReLU non-linearity. To aid regularization, we added batch normalization layers and dropout layers after the dense layers. We also applied l1 and l2 regularizers to all the dense layers to decrease overfitting. We set the the l1 regularization factor as 0.0001 and l2 regularization factor as 0.0005. Figure \ref{fig:Full system}(c) shows the complete network architecture of the base network, $VSBaseNet$.

\textbf{Integrated Approach:}
In this approach, the network directly outputs the actuations given an input image, $I$. For the integrated approach, the network used is $VSNet1$ which consists of the base network, $VSBaseNet$, along with a dense layer (output layer). Since we were dealing with a regression task, the final dense layer consisted of 5 units that output 5 floats corresponding to the 5 input actuations to the soft arm namely, bending ($b$), rotation ($r$), theta ($t$), and the gantry ($x$ and $y$). The details of $VSNet1$ are given in Figure \ref{fig:Full system}(b)   
 
\textbf{Modular Approach:}
For the modular approach, we divided the image-to-actuation step in two parts (modules): image-to-pose, and pose-to-actuation. The image-to-pose (Img2Pose) module takes in a single image (taken at the current arm  pose), $I$,  and  outputs  the pose information. The $VSBaseNet$ network is used to take an input image and output the pose in the  form  of  a  vector  comprising  of  the  position and orientation (quaternion) information, $(P_x, P_y, P_z,q_0, q_1, q_2, q_3)$. This pose information is fed as input to the $P2ANet$ network which predicts the corresponding mapping of actuation inputs in the form of another vector consisting of actuation values $(b, r, t, x, y)$. 

The network architecture of $VSBaseNet$ is similar to $VSNet1$ except the last (output) layer, which has 7 units corresponding to the 7 output floats. The $P2ANet$ consists of 3 dense layers with 256, 128, and 5 units respectively along with ReLU non-linearity. We also added batch normalization and dropout layers to aid regularization. The network architecture of $VSBaseNet$ and $P2ANet$ is given in Figure \ref{fig:Full system} part (b) and (d). 





\subsection{Training}

\subsubsection{Dataset}
A total of 7980 images corresponding to different poses were collected. The absolute pose data with respect to the initial configuration was noted for each of the images. We used electromagnetic tracking (Patriot SEU, Polhemus) with a short range source (TX1, tracking area 2 to 60 cm) to get the ground truth absolute pose. This sensor is flexible, lightweight ($<$ 2 g) and does not hinder or alter the performance of the soft arm. The sensor has a positional accuracy of less than 1
mm. The signal from the sensor provides the real time spatial coordinates of the soft arm end in the form of $[x,y,z,quaternion]$ and the angle and pressure inputs in the form of $[theta,r_1,r_2,b]$.\\
In our approach, we used image data to predict 5 actuation inputs to the soft arm. These actuation inputs are given by base angle $(theta)$, pressures $(r_1, r_2, b)$, and the gantry system configurations ($x, y$). For the purpose of training, we combined $r_1$ and $r_2$ into one actuation, $r$. The range of values for each of the 5 actuations were as follows: \\
Bending (\textit{b}): 14 to 22 psi; Rotation (\textit{r}): -18 to 18 psi; Theta (\textit{t}): +6 to -6 degrees; \textit{x}: 14, 16 and 18; \textit{y}: 14, 16 ,18,20.

We had a total of 7980 images in the dataset which we divided into training, validation and testing sets with 4910, 1676, and 2394 images respectively. 

\subsubsection{Ground Truth Label Description}
The ground truth values consisted of the absolute actuation values corresponding to the pose of the soft arm for each image. A CSV file containing 5 columns corresponding to each of the actuation values was created, and then split into training, validation and testing label files for training purposes. The entire method is automated.  

\subsection{Loss Function and Optimization}

Our network takes in a single image (taken at the current arm pose), \textit{I}, and outputs the absolute actuation values required to reach that pose. Since this is a regression problem, the last layer of the network outputs floats. The output of the network is in the form of a vector comprising of either the pose $(P_x, P_y, P_z,q_0, q_1, q_2, q_3)$ or the 5 actuations $(b, r, t, x, y)$. 

To regress absolute values of pose or actuations, we use the mean-squared error loss function which computes the mean of squared errors between the ground truth values and the predictions. 

\begin{equation}
    loss(I) = \frac{1}{n}\sum_{i=1}^{n}(Y_i - \hat{Y_i})^2 
\end{equation}

$Y_i$ corresponds to the ground truth actuations for the input image.  $\hat{Y_i}$ is the predicted actuations for the input image. 

The optimizer used in the training was Adam optimizer due to its fast converging properties. We used a time based learning rate scheduler with an initial learning rate of 0.01 and number of epochs as 150. The learning rate at each epoch was calculated as:
\begin{equation}
    \eta_{n} = \eta_{n-1} * \frac{1}{1+decay*n}
\end{equation}

where $\eta_{n-1}$ is the learning rate of the previous epoch, and $n$ is the current epoch number. The value of decay is normally implemented as:
\begin{equation}
    decay = \frac{\eta_0}{N}
\end{equation}

where $\eta_{n-1}$ is the initial learning rate and $N$ is the total number of epochs. We trained the model for 150 epochs after which the model reached saturation. We used a batch size of 128 to help in generalizing the model better. Using a lower or a higher batch size was causing the validation loss to fluctuate. 



\subsection{Control Law}
Due to the inherent non linearity of the SCA, effect of internal and external disturbances like weights the SCA may not necessarily reach the same pose when the training data is collected. IN addition, there will also be some errors due to the trained model. To overcome these unpredictable characteristics of the SCA behaviour we use a control law to make the tip of the SCA to converge to the target image ($I_T$). The following control law is used as shown in the Fig.\ref{fig:Full system}(a):
\begin{align}
    A_{RC}(k+1) = A_{RC}(k)-\lambda(A_{PC}(k)-A_{PT})
\end{align}
where $A_{RC}(k), A_{PC}(k) and A_{PT}$ are the current actuation's to the soft arm, predicted actuation's for the current image and predicted actuation's for the target image at step $k$. As the error between the predicted actuation's for the current image and target image reduces to zero the SCA reaches a steady state and also implies the tip is seeing the target image. $\lambda$ is the proportional gain ($> 0$) used for efficient convergence. 

